RLIP: Relational Language-Image Pre-training for Human-Object Interaction Detection

The task of Human-Object Interaction (HOI) detection targets fine-grained visual parsing of humans interacting with their environment, enabling a broad range of applications. Prior work has demonstrated the benefits of effective architecture design and integration of relevant cues for more accurate HOI detection. However, the design of an appropriate pre-training strategy for this task remains underexplored by existing approaches. To address this gap, we propose Relational Language-Image Pre-training (RLIP), a strategy for contrastive pre-training that leverages both entity and relation descriptions. To make effective use of such pre-training, we make three technical contributions: (1) a new Parallel entity detection and Sequential relation inference (ParSe) architecture that enables the use of both entity and relation descriptions during holistically optimized pre-training; (2) a synthetic data generation framework, Label Sequence Extension, that expands the scale of language data available within each minibatch; (3) mechanisms to account for ambiguity, Relation Quality Labels and Relation Pseudo-Labels, to mitigate the influence of ambiguous/noisy samples in the pre-training data. Through extensive experiments, we demonstrate the benefits of these contributions, collectively termed RLIP-ParSe, for improved zero-shot, few-shot and fine-tuning HOI detection performance as well as increased robustness to learning from noisy annotations. Code will be available at https://github.com/JacobYuan7/RLIP.

==> 06-checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{} It's mentioned in paragraph "\textbf{Leveraging off-the-shelf object detection data without relations}", and discussed in more detail in the supplementary material.
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{} It's included in the supplementary material.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} Data is publicly available and instructions are included in the experiment section.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)? 
    \answerYes{} They are included in Methodology and Experiments section. 
  \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{}
  \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{} It's included in the supplementary material.
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> paper/abstract.tex <==
\begin{abstract}
  The abstract paragraph should be indented \nicefrac{1}{2}~inch (3~picas) on
  both the left- and right-hand margins. Use 10~point type, with a vertical
  spacing (leading) of 11~points.  The word \textbf{Abstract} must be centered,
  bold, and in point size 12. Two line spaces precede the abstract. The abstract
  must be limited to one paragraph.
\end{abstract}

==> paper/introduction.tex <==

\section{Introduction}
% 第一段：基本背景
% 首先主要介绍之前的工作的主要任务是在模型架构的设计上（以DETR为基础的工作），忽略了初始化对于表示的重要性。

% 第二段：探索直接基于检测的初始化和基于relation的初始化，在特征表示上的区别（figure）。这种区别使得在relation inferring的时候，使用detection初始化是一sub-optimal的方式，由此引出pre-training with relations。

% 第三段：其次介绍HOI问题中open-world属性明显，zero-shot能力也会largely hinders its practicality，比如有些人的用词习惯就是不一样，词库也很小。
% 主体为现在的第三段，引出RLIP。

% 第四段：为了RLIP，设计了一个fully-disentangled架构。



%%%%%%
% Points to be discussed:
% 1. should I mention about decline of detection pretraining if pre-training on VG?
% 2. 用什么单词penalize regulate calibrate


%%% THis parahtaph aims to state some background information about HOI detection and introduce pre-training with relations.
Relation detection like human-object interaction (HOI) detection~\cite{chao2015hico} has been widely studied, aiming to detect triplets of the form <human, object, interactions>. An HOI detection system can serve as not only a tool for image/video data analysis by analysts in their own right, but also an essential building block for image/video captioning~\cite{yao2018exploringVR,pan2020STgraph_for_videocap}, image retrieval~\cite{johnson2015imageRt}, image synthesis~\cite{johnson2018imagegeneration_SG} and video action understanding~\cite{ji2020actiongenome}.

% 前人的工作关注在对于relation的定义上，于是设计了很多动词检测的架构，然而从没有人
HOI is a complex task with high semantic requirements, which can be composed of multiple functional components, such as detection, object classification, and relationship recognition, each of which has its own focus. Previous methods unify these disparate tasks within a single framework through an elaborate model structure design. These works are designing heuristic methods to infer relations between entities, spanning from interaction points~\cite{liao2020ppdm,zhong2021GGNet}, interaction boxes~\cite{kim2020uniondet}, contextualized embeddings~\cite{tamura2021qpic,kim2021hotr,zou2021HOITransformer,kim2021hotr}, poses~\cite{gupta2019nofrills,li2019interactiveness}, statistical priors~\cite{kim2020actioncooccur,Yuan2022OCN} to external knowledge like language embeddings \cite{Yuan2022OCN,xu2019HOIwithknowledge,peyre2019HOIwithanalogy}. 
Most of them paid little attention to the model initialization, which substantially impacts representation quality~\cite{dai2021updetr,zoph2020rethinking_pretrain}. 

\par

Recent pretraining-finetuning paradigm has made great strides in many fields, \textit{i.e.}, xx, xx,xx. 
From the perspective of the pretraining-finetuning paradigm, we find that there are two problems in the existing HOI methods, one is the misalignment of model features, and the other is the lack of open-set capability of features. For misalignment, A widely-adopted operation of fine-tuning an HOI detection model \cite{tamura2021qpic,Yuan2022OCN,chen2021ASNet,zou2021HOITransformer} is to initialize the relation inferring stage with parameters pre-trained on object detection tasks like COCO~\cite{lin2014MSCOCO}. From the perspective of attention maps, detection tasks are highly object-centered, while relation inferring are subject- and object-conditioned contextualized embeddings, indicating that detection parameters are possibly sub-optimal for conditional relation inferring. 
For open-set capability, any semantic-related task is inherently open-vocabulary~\cite{plummer2020open-ended_phrase_detection,zareian2021open_vocab}, in our case, meaning that people tend to use free-form texts to describe entities and relations, so as the annotation process, which results in that the number of latent categories of HOI is much larger than that in the training process during the application phase. Existing HOI methods overly rely on predetermined labels when learning representations, struggling to generalize to unseen concepts. 

\par
To tackle these mentioned problems, we propose a pretraining-finetuning paradigm for HOI task, RLIP(Relational Language-Image Pretraining). 





to align the pre-training phase with the fine-tuning phase by \textbf{pre-training with relations}.

Crowd-sourced datasets (\textit{e.g.} VG\cite{krishna2017visualgenome}) can provide abundant label sets defining visual concepts from entities to relations, without textual concepts pre-defined \cite{radford2021CLIP,li2021GLIP}. To make use of such relation-rich datasets for pre-training, a one-of-N objective is sub-optimal due to semantic similarity. Thus, we resort to language-image pre-training, which scales well to free-form concepts. Although there are works exploring to align image representations~\cite{radford2021CLIP,Jia2021ScalingUV} and regional representations~\cite{kamath2021MDETR,li2021GLIP} with free-form languages, explicit textual relations between regions are under-explored.
To fill this gap, we propose \textbf{Relational Language-Image Pre-training} (RLIP), aligning content-level object embeddings and context-level relational embeddings with corresponding free-form texts, which even equips an HOI detection model with a zero-shot ability\footnote{\textit{Zero-shot} means performing HOI detection without fine-tuning~\cite{radford2021CLIP}, an experiment setting that assesses a pre-training model's generalization to unseen distributions, which is different from the definition (unseen combinations or unseen objects) in previous HOI detection papers~\cite{hou2020VCL,hou2021FCL}}.
% Thus, we resolve it by introducing a language backbone (\textit{e.g.} RoBERTa~\cite{liu2019RoBERTa}) and explicitly aligning the relational texts with visual relational representations

Equipped with RLIP, one HOI detection model classifies one entity or relation by matching with languages rather than fixed-length learned weights. However, previous methods \cite{tamura2021qpic,Yuan2022OCN,chen2021qahoi,zou2021HOITransformer} use a coupled representation (\textit{i.e.} one feature for multiple entity/relation representations) for the subject, the object and the relation, which hinders its matching with their corresponding texts. 
To allow for a disentangled cross-modal matching, we propose ParSe based on DETR~\cite{carion2020DETR} or Deformable DETR (DDETR)~\cite{zhu2020deformableDETR} architecture, short for \textbf{Par}allel entity detection and \textbf{Se}quential relation inferring. ParSe's design is based on the independent entity assumption and conditional relation assumption. For the former, we define two group of queries respectively for subject and object content representations. For the latter, we generate conditional queries for relational context representations. ParSe achieves competitive results with uni-modal fine-tuning.

Building on ParSe, we design RLIP-ParSe that enables relational language-image pre-training. There are mainly two problems remaining to be solved: \textbf{i)} Captions usually do not exist for a relation detection dataset, on which a language-image pre-training relies. \textbf{ii)} Human-annotated labels intrinsically have semantic ambiguity, \textit{i.e.} entities or relations with identical semantic meanings have different labels, resulting in a large semantic-rich corpus. 
For the first obstacle, we introduce a permutable label sequence comprised of ground-truth labels extracted from an existing language backbone (\textit{e.g.} RoBERTa~\cite{liu2019RoBERTa}). While the size of the label set is intractable to handle, we aggregate in-batch labels and boost them with out-of-batch sampling to ensure a better language-image alignment. 
For the second obstacle, we take advantage of cross-modal data to ameliorate relational ambiguity. On the one hand, by incorporating the quality of the visual entity detection phase \cite{li2020GFLv1}, we calibrate the confidence of the relation matching its text label. On the other hand, by considering the similarities between labels within the label sequence, we extend relational labels for a given triplet via assigning pseudo soft labels.
% 用什么单词penalize regulate calibrate
% 但是问题有两个，一个是我们没有captions as previous language-image pre-training relying on complete captions~\cite{radford2021CLIP,kamath2021MDETR} or composed captions~\cite{li2021GLIP}，一个是我们组成了captions但是也suffer from semantic ambiguity. 为了解决第一个问题组成label sequence，label sequence带来的好处是我们既可以align in-batch的也可以align out of batch，为了解决第二个问题。我们怎么怎么semantic ambiguity problem and its solution: pseudo label and relation quality labels
% Unlike previous language-image pre-training that relies on complete captions~\cite{radford2021CLIP,kamath2021MDETR} or composed captions~\cite{li2021GLIP}, we introduce a label sequence comprised of ground-truth labels extracted from an existing language backbone (\textit{e.g.} RoBERTa~\cite{liu2019RoBERTa}). While the size of the label set is intractable to handle, we aggregate in-batch labels and boost them with out-of-batch sampling to ensure a better language-image alignment.
Experiments demonstrate that though pre-training on a noisy dataset, pre-training with relations can largely outperforms naive detection pre-training and is on par with pre-training on a elaborately-annotated object detection dataset like COCO~\cite{lin2014MSCOCO}. Moreover, RLIP-ParSe even surpasses several fully fine-tuning methods with mere zero-shot evaluation.

%%% This paragraph aims to summarize main contributions.





% which 让一个representation做multi-word matching，破坏性能。引用一些disentangled的文章，表示应该完全disentangled。
% Based on the previous motivation, we firstly propose a model termed  (ParSe), which disentangles the representations of the subject, the object and the relation in one triplet.

%  and scene graph generation (SGG)~\cite{xu2017iterative_message}

% 之前的relation detection的问题：
% 二阶段的检测器使用直接训练好的off-the-shelf detector，frozen
% 单阶段的不使用预训练或者使用COCO的预训练
% 单阶段的模型的性能越来越好，他们一部分是受益于COCO极好的标注，前人从来没有研究过，是否一个好的relation pre-training在类似的问题中也是必要的并且有用的呢？（加粗）
% （这里写的时候可以看一下我的PPT上是如何写的，借鉴一下。）


% 以下是我的部分想法：
% 不太成熟，有点问题
% One difference of DETR-based methods to traditional one-stage methods is its coupled representation for the localization and classification. In previous one-stage methods, methods like XXXXXX design ways to incorporate localization information into the classification branch.


==> paper/related.tex <==

\section{Related Work}
\paragraph{Human-Object Interaction Detection} Note: This paragraph aims to review methods on HOI detection, with an emphasis on methods that incorporates word embeddings and can perform zero-shot (different definition from ours as shown in introduction) HOI detection.

After DETR~\cite{carion2020DETR} is proposed, myriad model variants~\cite{Yuan2022OCN,zou2021HOITransformer,tamura2021qpic,chen2021ASNet,kim2021hotr,chen2021qahoi} have been proposed to tackle relation detection problem based on contextualized embeddings~\cite{tamura2021qpic}, generating considerable boosts.

% IDN is pre-training？because we are emphasizing the relational pre-training. 但是通过switch h或者o来训练一个classifier。


\paragraph{Language-Image Pre-training} Note: This paragraph aims to review related works about image-level and object-level cross-modal pre-training that ignores relational cues.

